The Early Ultraviolet Light-Curves of Type II Supernovae and the Radii of Their Progenitor Stars

We present a sample of 34 normal SNe II detected with the Zwicky Transient Facility, with multi-band UV light-curves starting at $t \leq 4$ days after explosion, as well as X-ray detections and upper limits. We characterize the early UV-optical colors and provide prescriptions for empirical host-extinction corrections. We show that the $t > 2\,$days UV-optical colors and the blackbody evolution of the sample are consistent with the predictions of spherical phase shock-cooling (SC), independently of the presence of `flash ionization" features. We present a framework for fitting SC models which can reproduce the parameters of a set of multi-group simulations without a significant bias up to 20% in radius and velocity. Observations of about half of the SNe II in the sample are well-fit by models with breakout radii $<10^{14}\,$cm. The other half are typically more luminous, with observations from day 1 onward that are better fit by a model with a large $>10^{14}\,$cm breakout radius. However, these fits predict an early rise during the first day that is too slow. We suggest these large-breakout events are explosions of stars with an inflated envelope or a confined CSM with a steep density profile, at which breakout occurs. Using the X-ray data, we derive constraints on the extended ($\sim10^{15}$ cm) CSM density independent of spectral modeling, and find most SNe II progenitors lose $<10^{-4} M_{\odot}\, \rm yr^{-1}$ a few years before explosion. This provides independent evidence the CSM around many SNe II progenitors is confined. We show that the overall observed breakout radius distribution is skewed to higher radii due to a luminosity bias. We argue that the $66^{+11}_{-22}\%$ of red supergiants (RSG) explode as SNe II with breakout radii consistent with the observed distribution of field RSG, with a tail extending to large radii, likely due to the presence of CSM.

==> results_table.tex <==
\begin{deluxetable*}{lcccccccc}
\centering
\label{tab:SC_res}
\tablecaption{Best fit parameters for shock cooling fitting}
\tablewidth{38pt} 
\hspace{3pt}
\tablehead{\colhead{SN} & \colhead{$R_{13}$} & \colhead{$v_{s*,8.5}$ } & \colhead{$f_{M}$} & \colhead{$E(B-V)$ [mag]} & \colhead{$R_{V}$} & \colhead{$t_{0}$ [JD]} & \colhead{$t_{0.7}$ [days]} & \colhead{$t_{tr}$ [days]}} 
\tabletypesize{\scriptsize} 
\startdata
SN2019eoh & $7.7^{+0.9}_{-0.9}$ & $2.0^{+0.3}_{-0.3}$ & $0.5^{+0.5}_{-0.4}$ & $0.0^{+0.0}_{-0.0}$ & $4.0^{+0.9}_{-1.3}$ & $-0.02^{+0.05}_{-0.06}$ & 26.7 & 16.3 \\
SN2020aavm & $13.4^{+4.1}_{-4.3}$ & $0.9^{+0.3}_{-0.3}$ & $83.7^{+85.7}_{-70.8}$ & $0.1^{+0.1}_{-0.1}$ & $3.9^{+1.0}_{-1.2}$ & $0.19^{+0.45}_{-0.50}$ & 22.2 & 47.1 \\
SN2020fqv & $3.4^{+1.6}_{-1.7}$ & $1.0^{+0.4}_{-0.3}$ & $99.4^{+76.4}_{-75.7}$ & $0.8^{+0.0}_{-0.0}$ & $2.8^{+0.5}_{-0.5}$ & $0.40^{+0.26}_{-0.28}$ & 13.8 & 47.4 \\
SN2019oxn & $5.4^{+0.8}_{-0.8}$ & $0.7^{+0.1}_{-0.1}$ & $1.4^{+1.7}_{-1.2}$ & $0.0^{+0.0}_{-0.0}$ & $3.9^{+0.9}_{-1.2}$ & $0.01^{+0.18}_{-0.21}$ & 20.2 & 46.8 \\
SN2020ufx & $15.2^{+3.8}_{-4.2}$ & $2.2^{+0.5}_{-0.4}$ & $83.0^{+81.7}_{-64.5}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.33^{+0.27}_{-0.33}$ & 27.7 & 4.6 \\
SN2019ozf & $16.5^{+2.8}_{-3.4}$ & $0.7^{+0.2}_{-0.2}$ & $94.5^{+77.6}_{-71.0}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.0}_{-1.2}$ & $-0.44^{+0.33}_{-0.33}$ & 20.6 & 30.9 \\
SN2018cxn & $13.7^{+3.2}_{-3.1}$ & $0.6^{+0.1}_{-0.1}$ & $109.7^{+68.1}_{-69.8}$ & $0.1^{+0.1}_{-0.1}$ & $3.8^{+1.0}_{-1.2}$ & $-0.00^{+0.01}_{-0.01}$ & 16.7 & 38.9 \\
SN2020cxd & $3.5^{+1.3}_{-1.0}$ & $0.3^{+0.1}_{-0.0}$ & $53.0^{+77.3}_{-47.4}$ & $0.1^{+0.1}_{-0.1}$ & $3.7^{+1.0}_{-1.2}$ & $0.48^{+0.53}_{-0.60}$ & 12.4 & 32.9 \\
SN2019nvm & $17.2^{+2.1}_{-2.2}$ & $0.7^{+0.1}_{-0.1}$ & $111.2^{+68.4}_{-70.3}$ & $0.1^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.1}$ & $-0.51^{+0.38}_{-0.34}$ & 25.6 & 38.2 \\
SN2020lfn & $17.5^{+2.1}_{-2.6}$ & $1.5^{+0.3}_{-0.2}$ & $98.5^{+72.3}_{-67.1}$ & $0.0^{+0.0}_{-0.0}$ & $3.8^{+1.0}_{-1.2}$ & $-0.24^{+0.22}_{-0.24}$ & 27.0 & 8.8 \\
SN2020jfo & $6.3^{+1.3}_{-1.3}$ & $0.6^{+0.1}_{-0.1}$ & $72.3^{+76.8}_{-56.8}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $0.11^{+0.23}_{-0.27}$ & 14.3 & 28.5 \\
SN2020nyb & $14.8^{+3.1}_{-3.0}$ & $0.4^{+0.1}_{-0.1}$ & $60.0^{+81.4}_{-53.1}$ & $0.1^{+0.1}_{-0.1}$ & $3.9^{+0.9}_{-1.1}$ & $-0.55^{+0.47}_{-0.60}$ & 21.9 & 60.6 \\
SN2019wzx & $14.0^{+4.9}_{-6.2}$ & $1.0^{+0.4}_{-0.3}$ & $92.6^{+79.7}_{-73.3}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.26^{+0.51}_{-0.55}$ & 20.2 & 31.2 \\
SN2019gmh & $14.9^{+4.6}_{-6.6}$ & $0.8^{+0.3}_{-0.2}$ & $132.4^{+55.0}_{-68.5}$ & $0.1^{+0.0}_{-0.0}$ & $4.1^{+0.7}_{-0.9}$ & $-0.30^{+0.20}_{-0.16}$ & 24.5 & 10.1 \\
SN2020afdi & $8.0^{+1.7}_{-1.6}$ & $0.4^{+0.1}_{-0.1}$ & $49.1^{+77.2}_{-45.2}$ & $0.0^{+0.0}_{-0.0}$ & $3.8^{+1.0}_{-1.2}$ & $-0.07^{+0.27}_{-0.28}$ & 21.8 & 48.5 \\
SN2020pqv & $17.3^{+2.2}_{-2.7}$ & $0.8^{+0.2}_{-0.2}$ & $80.0^{+83.6}_{-64.6}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.0}_{-1.2}$ & $-0.61^{+0.46}_{-0.50}$ & 29.5 & 13.5 \\
SN2020mst & $14.7^{+4.2}_{-4.5}$ & $0.9^{+0.2}_{-0.2}$ & $90.1^{+80.7}_{-72.2}$ & $0.1^{+0.1}_{-0.1}$ & $3.6^{+1.1}_{-1.2}$ & $-0.35^{+0.31}_{-0.33}$ & 24.6 & 23.6 \\
SN2020dyu & $16.0^{+3.2}_{-3.4}$ & $1.2^{+0.3}_{-0.2}$ & $105.0^{+71.6}_{-70.4}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.1}$ & $-0.54^{+0.28}_{-0.24}$ & 26.0 & 14.0 \\
SN2021apg & $14.9^{+3.9}_{-4.7}$ & $0.6^{+0.2}_{-0.2}$ & $87.9^{+80.8}_{-70.7}$ & $0.1^{+0.1}_{-0.1}$ & $3.7^{+1.0}_{-1.2}$ & $-0.31^{+0.76}_{-0.83}$ & 23.0 & 12.9 \\
SN2020xva & $10.6^{+3.0}_{-2.7}$ & $0.5^{+0.1}_{-0.1}$ & $66.8^{+84.8}_{-58.6}$ & $0.1^{+0.1}_{-0.1}$ & $4.0^{+0.8}_{-1.2}$ & $0.22^{+0.40}_{-0.46}$ & 18.6 & 44.5 \\
SN2020nif & $13.0^{+5.1}_{-5.0}$ & $1.6^{+0.4}_{-0.3}$ & $87.7^{+81.4}_{-70.5}$ & $0.1^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.07^{+0.41}_{-0.46}$ & 23.1 & 9.0 \\
SN2020acbm & $15.5^{+2.3}_{-2.4}$ & $0.7^{+0.1}_{-0.1}$ & $92.6^{+77.5}_{-70.7}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.1}_{-1.2}$ & $-0.46^{+0.33}_{-0.33}$ & 26.7 & 10.8 \\
SN2021yja & $15.2^{+3.8}_{-4.6}$ & $0.6^{+0.2}_{-0.1}$ & $90.2^{+80.7}_{-72.7}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $0.39^{+1.08}_{-1.08}$ & 21.7 & 54.2 \\
SN2019omp & $13.5^{+4.9}_{-5.0}$ & $0.8^{+0.2}_{-0.2}$ & $105.5^{+72.9}_{-74.3}$ & $0.1^{+0.1}_{-0.1}$ & $3.7^{+1.0}_{-1.2}$ & $-0.48^{+0.33}_{-0.31}$ & 24.4 & 33.1 \\
SN2021ibn & $8.0^{+2.8}_{-2.6}$ & $1.9^{+0.5}_{-0.5}$ & $89.1^{+80.3}_{-69.5}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.0}_{-1.2}$ & $0.19^{+0.15}_{-0.18}$ & 17.6 & 6.8 \\
SN2020qvw & $15.2^{+3.7}_{-4.4}$ & $1.4^{+0.3}_{-0.3}$ & $90.1^{+80.7}_{-70.3}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.10^{+0.25}_{-0.21}$ & 24.0 & 6.5 \\
SN2018fif & $12.2^{+3.5}_{-3.3}$ & $0.7^{+0.1}_{-0.1}$ & $63.8^{+79.4}_{-54.2}$ & $0.2^{+0.1}_{-0.1}$ & $4.2^{+0.6}_{-0.9}$ & $-0.25^{+0.22}_{-0.29}$ & 20.6 & 47.2 \\
SN2020pni & $14.8^{+4.2}_{-5.1}$ & $1.4^{+0.5}_{-0.4}$ & $92.3^{+79.0}_{-71.1}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.0}_{-1.2}$ & $0.14^{+0.73}_{-0.68}$ & 25.5 & 10.8 \\
SN2021skn & $12.8^{+5.4}_{-5.0}$ & $1.1^{+0.4}_{-0.3}$ & $105.7^{+71.5}_{-73.3}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.48^{+0.38}_{-0.32}$ & 23.3 & 10.8 \\
SN2020uim & $13.4^{+1.8}_{-1.7}$ & $0.4^{+0.1}_{-0.1}$ & $52.7^{+79.2}_{-47.6}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.1}_{-1.2}$ & $-0.24^{+0.30}_{-0.37}$ & 20.7 & 55.0 \\
SN2018dfc & $15.1^{+4.0}_{-4.7}$ & $1.4^{+0.5}_{-0.4}$ & $105.5^{+71.7}_{-72.1}$ & $0.0^{+0.0}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $-0.76^{+0.29}_{-0.23}$ & 27.8 & 13.7 \\
SN2020xhs & $14.1^{+3.3}_{-3.7}$ & $0.5^{+0.2}_{-0.1}$ & $96.4^{+78.4}_{-75.3}$ & $0.1^{+0.1}_{-0.0}$ & $3.6^{+1.1}_{-1.2}$ & $0.59^{+0.61}_{-0.51}$ & 19.5 & 49.9 \\
SN2019ust & $10.0^{+2.2}_{-2.1}$ & $2.1^{+0.4}_{-0.4}$ & $17.1^{+24.9}_{-15.7}$ & $0.2^{+0.0}_{-0.0}$ & $4.1^{+0.7}_{-0.9}$ & $0.57^{+0.12}_{-0.14}$ & 23.1 & 4.8 \\
SN2020abue & $13.9^{+3.0}_{-3.0}$ & $0.6^{+0.1}_{-0.1}$ & $97.0^{+77.3}_{-73.6}$ & $0.0^{+0.0}_{-0.0}$ & $3.7^{+1.1}_{-1.2}$ & $-0.86^{+0.50}_{-0.48}$ & 22.5 & 26.8 \\
\enddata
\tablenotetext{a}{all times are in rest-frame days}
\tablenotetext{b}{Uncertainties reflect the 10th-90th percentiles of the posterior probability distribution}
\tablenotetext{c}{This table will be made available in machine-readable format through the journal website upon publication.}
\end{deluxetable*}


==> tab_XRT.tex <==
\begin{deluxetable*}{ccccccc}
\centering
\label{tab:XRT}
\tablecaption{XRT photometry for SNe included in this study}
\tablewidth{34pt} 
\tablehead{\colhead{SN} &\colhead{$t$ [day]} & \colhead{ $t_{\rm max}$ [day]} & \colhead{$t_{\rm min}$ [day]} & \colhead{XRT count rate [s$^{-1}$]} & \colhead{Flux [$10^{-14}$ erg s$^{-1}$ cm$^{-2}$]} & \colhead{Luminosity [$10^{40}$ erg s$^{-1}$]}} 
\tabletypesize{\scriptsize} 
\startdata
SN\,2018cxn & 7.2 & 10.0 & 1.6 & $<0.002$ & $<7.1$ & $<28.3$ \\
SN\,2018dfc & 1.5 & 5.2 & 1.5 & $<0.0011$ & $<4.3$ & $<14.08$ \\
SN\,2018fif & 2.1 & 16.8 & 1.2 & $<0.0015$ & $<6.4$ & $<4.56$ \\
SN\,2019eoh & 11.6 & 20.0 & 1.4 & $<0.0015$ & $<5.3$ & $<33.68$ \\
SN\,2019gmh & 479.9 & 480.4 & 1.9 & $<0.0009$ & $<3.2$ & $<7.41$ \\
SN\,2019nvm & 7.6 & 230.2 & 0.3 & $<0.0006$ & $<2.3$ & $<1.85$ \\
SN\,2019omp & 2.6 & 11.2 & 1.8 & $<0.0019$ & $<6.9$ & $<35.07$ \\
SN\,2019oxn & 2.3 & 10.6 & 0.7 & $<0.0018$ & $<6.8$ & $<6.6$ \\
SN\,2019ozf & 196.6 & 391.3 & 1.9 & $<0.0005$ & $<1.9$ & $<10.9$ \\
SN\,2019ust & 20.5 & 325.5 & 2.1 & $<0.0005$ & $<2.2$ & $<2.55$ \\
SN\,2019wzx & 28.7 & 692.5 & 2.1 & $<0.0008$ & $<2.9$ & $<5.39$ \\
SN\,2020aavm & 4.3 & 6.2 & 2.4 & $<0.0016$ & $<6.2$ & $<31.65$ \\
SN\,2020abue & 1.7 & 11.3 & 0.4 & $<0.0018$ & $<7.0$ & $<13.45$ \\
SN\,2020acbm & 5.7 & 22.8 & 0.3 & $0.0011 \pm 0.0004$ & $4.0 \pm 1.5$ & $4.56 \pm 1.71$ \\
SN\,2020afdi & 3.2 & 4.0 & 2.3 & $<0.0027$ & $<10.1$ & $<14.05$ \\
SN\,2020cxd & 5.0 & 14.9 & 2.9 & $<0.0028$ & $<10.7$ & $<0.38$ \\
SN\,2020dyu & 9.6 & 476.7 & 2.3 & $<0.0008$ & $<2.9$ & $<18.22$ \\
SN\,2020fqv & 1.7 & 59.0 & 0.0 & $<0.0072$ & $<43.1$ & $<5.79$ \\
SN\,2020jfo & 1.4 & 84.5 & 0.0 & $<0.0017$ & $<6.3$ & $<0.41$ \\
SN\,2020lfn & 4.0 & 119.5 & 1.4 & $<0.0004$ & $<1.7$ & $<8.03$ \\
SN\,2020mst & 2.4 & 13.5 & 1.4 & $<0.0013$ & $<5.2$ & $<46.13$ \\
SN\,2020nif & 3.3 & 16.8 & 0.0 & $<0.006$ & $<22.9$ & $<5.87$ \\
SN\,2020nyb & 4.2 & 12.3 & 1.2 & $<0.0012$ & $<5.3$ & $<3.05$ \\
SN\,2020pni & 6.9 & 103.1 & 0.6 & $<0.0006$ & $<2.1$ & $<1.41$ \\
SN\,2020pqv & 12.6 & 31.3 & 1.5 & $0.0005 \pm 0.0002$ & $1.8 \pm 0.9$ & $5.2 \pm 2.42$ \\
SN\,2020qvw & 3.7 & 484.5 & 2.6 & $<0.0016$ & $<6.2$ & $<39.45$ \\
SN\,2020ufx & 2.7 & 267.2 & 1.7 & $<0.0007$ & $<2.8$ & $<17.74$ \\
SN\,2020uim & 272.2 & 272.5 & 272.0 & $<0.0036$ & $<14.7$ & $<12.14$ \\
SN\,2020uim & 10.0 & 271.8 & 1.6 & $0.0008 \pm 0.0004$ & $3.1 \pm 1.5$ & $2.6 \pm 1.26$ \\
SN\,2020xhs & 17.5 & 256.7 & 2.6 & $<0.0014$ & $<6.3$ & $<9.06$ \\
SN\,2020xva & 2.0 & 18.3 & 1.9 & $<0.0009$ & $<3.5$ & $<4.92$ \\
SN\,2021apg & 8.1 & 14.3 & 1.9 & $<0.0014$ & $<4.8$ & $<8.53$ \\
SN\,2021ibn & 129.6 & 257.3 & 1.9 & $<0.0008$ & $<2.8$ & $<13.54$ \\
SN\,2021skn & 2.8 & 12.1 & 1.4 & $<0.0015$ & $<5.4$ & $<11.68$ \\
SN\,2021yja & 4.3 & 8.0 & 2.3 & $0.0013 \pm 0.0003$ & $4.8 \pm 1.2$ & $0.32 \pm 0.08$ \\
SN\,2021yja & 46.9 & 83.2 & 15.9 & $<0.0006$ & $<2.1$ & $<0.14$ \\
\hline
\enddata
\tablenotetext{a}{All times are reported in rest-frame days}
\tablenotetext{b}{We report 3$\sigma$ upper limits, or measurements with a significance of 3$\sigma$ above the background level. }
\tablenotetext{c}{Fluxes are corrected for galactic neutral hydrogen column density, and converted from count-rates assuming a power-law spectrum with a photon index of 2.}
\tablenotetext{d}{For SN\,2020jfo, SN\,2020fqv and SN\,2020nif we report quiescent host-galaxy detections as upper limits on the SN flux.}
\end{deluxetable*}

==> tab_bb_full.tex <==
\begin{deluxetable*}{lcccccccc}
\label{tab:bb_trunc}
\centering
\tablecaption{Early-time blackbody fits of SNe included in this work (truncated)}
\tablewidth{34pt} 
\tablehead{\colhead{SN} & \colhead{t [rest-frame days]} & \colhead{$\rm T_{eff}\ [K]$} & \colhead{$\rm R_{BB}\ [10^{14} \rm cm]$ } & \colhead{$\rm L_{pseudo}\ [10^{42} \rm erg\ \rm s^{-1}]$} & \colhead{$\rm L_{pseudo,extrap}\  [10^{42} \rm erg\ \rm s^{-1}]$}& \colhead{$\chi^{2}/dof$}  } 
\tabletypesize{\scriptsize} 
\startdata
SN2018cxn & 1.6 & $23500\pm1500$ & $2.15\pm0.16$ & $3.749\pm0.009$ & $10.0\pm0.7$ & 1.4 \\
SN2018cxn & 2.19 & $20800\pm1400$ & $2.58\pm0.22$ & $3.767\pm0.009$ & $8.7\pm0.5$ & 2.2 \\
SN2018cxn & 5.6 & $12700\pm600$ & $5.3\pm0.42$ & $3.497\pm0.007$ & $5.1\pm0.1$ & 2.0 \\
SN2018cxn & 9.59 & $10500\pm300$ & $6.82\pm0.34$ & $2.827\pm0.007$ & $3.88\pm0.04$ & 0.6 \\
SN2018dfc & 1.58 & $22000\pm800$ & $4.31\pm0.2$ & $13.18\pm0.02$ & $31.0\pm1.0$ & 1.0 \\
SN2018dfc & 3.19 & $17000\pm500$ & $5.99\pm0.25$ & $12.46\pm0.02$ & $21.7\pm0.4$ & 1.0 \\
SN2018dfc & 4.1 & $15000\pm300$ & $6.92\pm0.21$ & $10.69\pm0.02$ & $17.1\pm0.2$ & 0.5 \\
SN2018dfc & 5.03 & $13300\pm200$ & $8.19\pm0.29$ & $9.88\pm0.02$ & $14.7\pm0.1$ & 0.5 \\
SN2018fif & 1.22 & $20600\pm1500$ & $1.68\pm0.14$ & $1.671\pm0.003$ & $3.7\pm0.3$ & 2.7 \\
SN2018fif & 1.25 & $20100\pm1100$ & $1.73\pm0.12$ & $1.646\pm0.003$ & $3.5\pm0.2$ & 2.1 \\
SN2018fif & 2.1 & $15600\pm500$ & $2.7\pm0.15$ & $1.851\pm0.003$ & $3.08\pm0.06$ & 1.6 \\
SN2018fif & 2.65 & $15100\pm700$ & $2.87\pm0.21$ & $1.813\pm0.003$ & $2.96\pm0.07$ & 2.9 \\
SN2018fif & 4.57 & $12000\pm600$ & $4.22\pm0.3$ & $1.976\pm0.003$ & $2.65\pm0.05$ & 3.6 \\
SN2018fif & 6.15 & $11200\pm600$ & $4.86\pm0.42$ & $2.041\pm0.003$ & $2.68\pm0.05$ & 4.4 \\
SN2018fif & 6.17 & $11100\pm600$ & $4.87\pm0.42$ & $2.042\pm0.003$ & $2.68\pm0.05$ & 4.4 \\
SN2018fif & 7.31 & $10600\pm600$ & $5.33\pm0.46$ & $2.037\pm0.003$ & $2.66\pm0.04$ & 4.2 \\
SN2018fif & 8.33 & $10000\pm500$ & $5.86\pm0.49$ & $1.997\pm0.004$ & $2.6\pm0.04$ & 3.5 \\
SN2018fif & 9.37 & $8600\pm400$ & $7.48\pm0.55$ & $1.628\pm0.004$ & $2.26\pm0.03$ & 1.6 \\
SN2018fif & 14.4 & $7700\pm200$ & $9.21\pm0.44$ & $1.573\pm0.003$ & $2.18\pm0.02$ & 0.9 \\
SN2018fif & 15.12 & $7600\pm200$ & $9.47\pm0.35$ & $1.536\pm0.004$ & $2.15\pm0.01$ & 0.5 \\
SN2018fif & 16.67 & $7100\pm100$ & $10.42\pm0.29$ & $1.286\pm0.003$ & $1.974\pm0.009$ & 0.3 \\
SN2019eoh & 1.46 & $24400\pm500$ & $2.59\pm0.07$ & $6.5\pm0.01$ & $16.9\pm0.4$ & 0.2 \\
SN2019eoh & 2.27 & $25000\pm800$ & $3.07\pm0.12$ & $9.76\pm0.02$ & $26.0\pm1.0$ & 0.6 \\
SN2019eoh & 3.09 & $21500\pm900$ & $3.74\pm0.2$ & $9.8\pm0.02$ & $21.3\pm0.9$ & 1.5 \\
SN2019eoh & 4.36 & $19500\pm700$ & $4.44\pm0.23$ & $10.97\pm0.02$ & $20.6\pm0.6$ & 1.7 \\
SN2019eoh & 5.96 & $16800\pm800$ & $5.46\pm0.34$ & $10.2\pm0.02$ & $16.8\pm0.5$ & 2.5 \\
SN2019eoh & 9.32 & $12100\pm400$ & $8.22\pm0.43$ & $7.47\pm0.01$ & $10.0\pm0.1$ & 1.9 \\
SN2019eoh & 11.04 & $10400\pm300$ & $9.92\pm0.45$ & $6.49\pm0.01$ & $8.33\pm0.07$ & 1.0 \\
SN2019eoh & 12.61 & $10000\pm200$ & $10.32\pm0.42$ & $5.95\pm0.01$ & $7.66\pm0.06$ & 0.8 \\
SN2019eoh & 14.38 & $9200\pm300$ & $11.28\pm0.56$ & $4.66\pm0.01$ & $6.34\pm0.07$ & 0.8 \\
SN2019eoh & 14.92 & $9000\pm300$ & $11.68\pm0.71$ & $4.47\pm0.01$ & $6.1\pm0.07$ & 1.1 \\
SN2019gmh & 1.9 & $18000\pm600$ & $3.25\pm0.16$ & $4.218\pm0.008$ & $8.0\pm0.2$ & 1.3 \\
SN2019gmh & 3.08 & $15400\pm500$ & $3.99\pm0.22$ & $3.966\pm0.009$ & $6.4\pm0.1$ & 1.6 \\
SN2019gmh & 4.04 & $13700\pm400$ & $4.67\pm0.23$ & $4.215\pm0.009$ & $5.81\pm0.08$ & 1.8 \\
SN2019gmh & 4.91 & $12300\pm400$ & $5.38\pm0.24$ & $3.817\pm0.01$ & $4.99\pm0.06$ & 1.1 \\
SN2019gmh & 5.72 & $11100\pm200$ & $6.19\pm0.23$ & $3.664\pm0.008$ & $4.61\pm0.03$ & 0.9 \\
SN2019nvm & 0.36 & $24000\pm1300$ & $2.39\pm0.14$ & $4.888\pm0.007$ & $13.5\pm0.9$ & 2.1 \\
SN2019nvm & 1.45 & $16600\pm400$ & $3.95\pm0.13$ & $5.006\pm0.006$ & $8.2\pm0.1$ & 1.5 \\
SN2019nvm & 2.29 & $16200\pm400$ & $4.17\pm0.14$ & $5.244\pm0.008$ & $8.4\pm0.2$ & 1.5 \\
SN2019nvm & 4.22 & $12800\pm400$ & $5.58\pm0.26$ & $4.129\pm0.005$ & $5.68\pm0.08$ & 3.6 \\
SN2019nvm & 10.38 & $9700\pm600$ & $7.64\pm0.81$ & $2.845\pm0.005$ & $3.67\pm0.08$ & 11.1 \\
SN2019nvm & 12.33 & $9500\pm600$ & $7.88\pm0.79$ & $2.959\pm0.006$ & $3.76\pm0.08$ & 8.7 \\
SN2019nvm & 14.09 & $9100\pm700$ & $8.24\pm0.99$ & $2.51\pm0.005$ & $3.35\pm0.09$ & 9.9 \\
SN2019nvm & 18.27 & $8300\pm800$ & $9.24\pm1.5$ & $1.983\pm0.004$ & $2.9\pm0.1$ & 13.6 \\
SN2019nvm & 21.2 & $8000\pm800$ & $9.53\pm1.63$ & $1.863\pm0.004$ & $2.69\pm0.1$ & 13.3 \\
SN2019nvm & 26.03 & $7600\pm900$ & $10.16\pm2.08$ & $1.523\pm0.003$ & $2.3\pm0.1$ & 16.0 \\
SN2019nvm & 26.64 & $7700\pm900$ & $10.0\pm2.04$ & $1.65\pm0.003$ & $2.4\pm0.1$ & 16.6 \\
SN2019nvm & 29.47 & $8900\pm1900$ & $7.94\pm2.43$ & $1.086\pm0.002$ & $2.9\pm0.4$ & 15.6 \\
SN2019omp & 1.84 & $17600\pm800$ & $3.3\pm0.22$ & $4.34\pm0.01$ & $7.5\pm0.2$ & 1.6 \\
SN2019omp & 3.08 & $15500\pm400$ & $4.05\pm0.18$ & $4.474\pm0.009$ & $6.74\pm0.1$ & 0.8 \\
SN2019omp & 4.0 & $13700\pm400$ & $4.88\pm0.22$ & $4.23\pm0.01$ & $5.91\pm0.07$ & 0.8 \\
SN2019omp & 6.52 & $10800\pm500$ & $6.84\pm0.49$ & $3.609\pm0.01$ & $4.61\pm0.06$ & 1.7 \\
SN2019omp & 10.96 & $8200\pm200$ & $10.65\pm0.36$ & $2.525\pm0.008$ & $3.67\pm0.02$ & 0.1 \\
SN2019oxn & 0.77 & $26500\pm1100$ & $0.98\pm0.04$ & $1.091\pm0.002$ & $3.4\pm0.2$ & 0.4 \\
SN2019oxn & 2.49 & $19800\pm800$ & $1.64\pm0.09$ & $1.472\pm0.003$ & $3.0\pm0.1$ & 1.3 \\
SN2019oxn & 3.18 & $18100\pm600$ & $1.87\pm0.08$ & $1.492\pm0.003$ & $2.71\pm0.07$ & 1.1 \\
SN2019oxn & 4.61 & $14800\pm400$ & $2.44\pm0.1$ & $1.387\pm0.003$ & $2.07\pm0.03$ & 0.8 \\
SN2019oxn & 5.19 & $13700\pm400$ & $2.72\pm0.12$ & $1.345\pm0.004$ & $1.89\pm0.03$ & 0.9 \\
SN2019oxn & 7.53 & $12200\pm200$ & $3.2\pm0.11$ & $1.306\pm0.003$ & $1.71\pm0.01$ & 0.6 \\
SN2019oxn & 8.06 & $12100\pm300$ & $3.2\pm0.13$ & $1.216\pm0.003$ & $1.61\pm0.02$ & 0.8 \\
SN2019oxn & 9.63 & $10000\pm400$ & $4.08\pm0.26$ & $0.931\pm0.002$ & $1.19\pm0.01$ & 1.7 \\
SN2019oxn & 10.5 & $10200\pm300$ & $3.92\pm0.17$ & $0.989\pm0.002$ & $1.247\pm0.009$ & 0.8 \\
SN2019ozf & 1.95 & $20800\pm1000$ & $3.03\pm0.17$ & $5.76\pm0.01$ & $12.3\pm0.5$ & 0.9 \\
SN2019ozf & 2.91 & $16800\pm400$ & $4.07\pm0.12$ & $5.41\pm0.01$ & $9.4\pm0.1$ & 0.3 \\
SN2019ozf & 3.87 & $17100\pm800$ & $4.23\pm0.3$ & $5.69\pm0.02$ & $10.3\pm0.4$ & 1.5 \\
SN2019ozf & 4.78 & $14700\pm500$ & $5.12\pm0.28$ & $5.77\pm0.01$ & $8.9\pm0.2$ & 1.1 \\
SN2019ozf & 6.21 & $12400\pm700$ & $6.34\pm0.59$ & $4.56\pm0.01$ & $6.7\pm0.2$ & 1.9 \\
SN2019ozf & 7.29 & $11800\pm400$ & $6.91\pm0.36$ & $4.46\pm0.01$ & $6.42\pm0.08$ & 0.7 \\
SN2019ozf & 7.98 & $11700\pm500$ & $7.09\pm0.47$ & $5.44\pm0.01$ & $7.0\pm0.1$ & 1.7 \\
SN2019ozf & 9.13 & $11500\pm500$ & $7.02\pm0.4$ & $4.75\pm0.01$ & $6.14\pm0.08$ & 0.7 \\
SN2019ozf & 9.91 & $10800\pm400$ & $7.46\pm0.38$ & $4.11\pm0.01$ & $5.3\pm0.06$ & 0.4 \\
SN2019ust & 2.08 & $17300\pm1200$ & $3.24\pm0.33$ & $3.738\pm0.007$ & $6.8\pm0.3$ & 3.8 \\
SN2019ust & 3.42 & $15900\pm1600$ & $4.29\pm0.62$ & $5.153\pm0.007$ & $8.5\pm0.5$ & 13.0 \\
SN2019ust & 5.5 & $13400\pm800$ & $5.93\pm0.52$ & $6.468\pm0.008$ & $8.6\pm0.2$ & 8.6 \\
SN2019ust & 6.58 & $12300\pm700$ & $6.8\pm0.58$ & $6.17\pm0.01$ & $7.8\pm0.2$ & 6.1 \\
SN2019ust & 14.36 & $8600\pm100$ & $11.85\pm0.27$ & $4.527\pm0.006$ & $5.59\pm0.02$ & 0.7 \\
SN2019ust & 16.47 & $7900\pm100$ & $13.26\pm0.39$ & $3.762\pm0.005$ & $4.81\pm0.02$ & 1.0 \\
SN2019ust & 18.84 & $7500\pm100$ & $14.51\pm0.53$ & $3.595\pm0.005$ & $4.67\pm0.03$ & 1.5 \\
SN2019ust & 20.54 & $7200\pm200$ & $15.02\pm0.7$ & $3.271\pm0.004$ & $4.34\pm0.03$ & 2.1 \\
SN2019ust & 22.33 & $7000\pm200$ & $15.42\pm0.79$ & $3.003\pm0.004$ & $4.06\pm0.03$ & 2.1 \\
SN2019wzx & 2.15 & $24700\pm1500$ & $2.69\pm0.2$ & $7.27\pm0.01$ & $20.0\pm1.0$ & 2.0 \\
SN2019wzx & 4.42 & $17900\pm1200$ & $3.91\pm0.37$ & $7.01\pm0.01$ & $12.2\pm0.5$ & 4.7 \\
SN2019wzx & 5.4 & $15700\pm1000$ & $4.62\pm0.45$ & $6.607\pm0.009$ & $10.3\pm0.3$ & 5.8 \\
SN2019wzx & 7.65 & $12300\pm600$ & $6.42\pm0.6$ & $5.265\pm0.009$ & $7.4\pm0.1$ & 5.1 \\
SN2019wzx & 12.25 & $9000\pm300$ & $10.66\pm0.83$ & $3.648\pm0.006$ & $5.57\pm0.09$ & 2.2 \\
SN2019wzx & 15.0 & $7900\pm300$ & $13.37\pm1.18$ & $3.026\pm0.006$ & $5.04\pm0.1$ & 1.5 \\
SN2020aavm & 2.46 & $23700\pm1700$ & $2.5\pm0.23$ & $5.22\pm0.01$ & $14.0\pm1.0$ & 1.6 \\
SN2020aavm & 3.05 & $21100\pm1000$ & $2.86\pm0.18$ & $5.1\pm0.01$ & $11.4\pm0.5$ & 0.8 \\
SN2020aavm & 4.17 & $19200\pm300$ & $3.28\pm0.07$ & $5.44\pm0.01$ & $10.6\pm0.1$ & 0.1 \\
SN2020aavm & 4.99 & $17700\pm900$ & $3.57\pm0.25$ & $4.67\pm0.01$ & $8.6\pm0.3$ & 1.1 \\
SN2020aavm & 5.09 & $17500\pm900$ & $3.61\pm0.25$ & $4.66\pm0.01$ & $8.5\pm0.3$ & 1.1 \\
SN2020aavm & 5.73 & $16500\pm500$ & $3.87\pm0.17$ & $4.48\pm0.01$ & $7.7\pm0.1$ & 0.5 \\
SN2020abue & 0.45 & $25800\pm2100$ & $1.96\pm0.18$ & $4.103\pm0.008$ & $12.0\pm1.0$ & 2.2 \\
SN2020abue & 1.54 & $21100\pm1200$ & $2.61\pm0.2$ & $4.351\pm0.007$ & $9.7\pm0.5$ & 2.1 \\
SN2020abue & 2.7 & $17300\pm800$ & $3.42\pm0.23$ & $4.413\pm0.008$ & $7.7\pm0.2$ & 2.3 \\
SN2020abue & 3.47 & $15500\pm600$ & $4.02\pm0.23$ & $4.4\pm0.01$ & $7.0\pm0.2$ & 1.4 \\
SN2020abue & 6.22 & $12200\pm300$ & $5.67\pm0.27$ & $3.655\pm0.006$ & $5.21\pm0.05$ & 1.4 \\
SN2020abue & 11.11 & $9300\pm300$ & $8.5\pm0.5$ & $2.895\pm0.007$ & $4.15\pm0.05$ & 1.2 \\
SN2020acbm & 0.74 & $28600\pm2200$ & $2.06\pm0.15$ & $5.821\pm0.01$ & $20.0\pm3.0$ & 2.7 \\
SN2020acbm & 0.75 & $28400\pm2200$ & $2.08\pm0.15$ & $5.832\pm0.01$ & $20.0\pm3.0$ & 2.9 \\
SN2020acbm & 1.62 & $23300\pm800$ & $2.77\pm0.11$ & $6.66\pm0.01$ & $16.5\pm0.7$ & 1.1 \\
SN2020acbm & 3.74 & $16600\pm500$ & $4.37\pm0.18$ & $6.539\pm0.01$ & $10.5\pm0.2$ & 1.7 \\
SN2020acbm & 4.81 & $14800\pm400$ & $5.08\pm0.18$ & $6.532\pm0.009$ & $9.3\pm0.1$ & 1.4 \\
SN2020acbm & 8.87 & $11300\pm400$ & $7.17\pm0.33$ & $4.398\pm0.007$ & $6.37\pm0.1$ & 1.1 \\
SN2020acbm & 16.89 & $8800\pm400$ & $9.61\pm0.69$ & $2.992\pm0.007$ & $4.04\pm0.05$ & 1.7 \\
SN2020acbm & 19.11 & $8900\pm600$ & $9.38\pm0.97$ & $2.207\pm0.007$ & $3.9\pm0.1$ & 1.7 \\
SN2020acbm & 20.86 & $8800\pm700$ & $9.46\pm1.15$ & $1.62\pm0.004$ & $3.8\pm0.2$ & 2.2 \\
SN2020acbm & 22.73 & $8300\pm700$ & $10.01\pm1.42$ & $1.527\pm0.003$ & $3.5\pm0.2$ & 3.1 \\
SN2020afdi & 2.29 & $20000\pm400$ & $1.66\pm0.05$ & $1.506\pm0.004$ & $3.09\pm0.06$ & 0.3 \\
SN2020afdi & 2.69 & $18200\pm600$ & $1.79\pm0.08$ & $1.414\pm0.004$ & $2.56\pm0.06$ & 0.7 \\
SN2020afdi & 3.29 & $16400\pm800$ & $1.96\pm0.12$ & $1.408\pm0.005$ & $2.18\pm0.06$ & 1.1 \\
SN2020afdi & 3.87 & $15000\pm800$ & $2.2\pm0.16$ & $1.274\pm0.005$ & $1.86\pm0.05$ & 1.3 \\
SN2020afdi & 5.82 & $9700\pm300$ & $3.87\pm0.15$ & $0.2575\pm0.0004$ & $0.94\pm0.02$ & 0.1 \\
SN2020afdi & 8.75 & $9100\pm500$ & $4.13\pm0.32$ & $0.2458\pm0.0004$ & $0.85\pm0.04$ & 0.3 \\
SN2020cxd & 3.2 & $12000\pm300$ & $1.43\pm0.05$ & $0.2478\pm0.0004$ & $0.316\pm0.003$ & 1.2 \\
SN2020cxd & 5.71 & $10000\pm400$ & $1.78\pm0.11$ & $0.1173\pm0.0003$ & $0.226\pm0.006$ & 0.7 \\
SN2020cxd & 10.82 & $9000\pm700$ & $2.03\pm0.24$ & $0.1069\pm0.0003$ & $0.189\pm0.008$ & 2.6 \\
SN2020cxd & 13.43 & $9100\pm800$ & $1.96\pm0.26$ & $0.0766\pm0.0001$ & $0.19\pm0.01$ & 2.7 \\
SN2020cxd & 15.12 & $8700\pm800$ & $2.04\pm0.29$ & $0.0752\pm0.0001$ & $0.18\pm0.01$ & 3.1 \\
SN2020dyu & 3.79 & $17000\pm600$ & $5.42\pm0.25$ & $11.75\pm0.02$ & $18.4\pm0.5$ & 2.3 \\
SN2020dyu & 4.51 & $17300\pm500$ & $5.29\pm0.22$ & $10.99\pm0.02$ & $17.9\pm0.4$ & 1.9 \\
SN2020dyu & 6.7 & $14600\pm400$ & $6.17\pm0.26$ & $9.17\pm0.02$ & $12.8\pm0.2$ & 2.0 \\
SN2020dyu & 7.64 & $13900\pm600$ & $6.64\pm0.38$ & $8.76\pm0.02$ & $11.8\pm0.2$ & 3.7 \\
SN2020dyu & 8.59 & $13100\pm600$ & $6.96\pm0.45$ & $8.73\pm0.02$ & $11.2\pm0.2$ & 3.2 \\
SN2020dyu & 9.6 & $12600\pm600$ & $7.27\pm0.5$ & $7.1\pm0.01$ & $9.7\pm0.2$ & 3.7 \\
SN2020dyu & 16.25 & $9300\pm400$ & $10.55\pm0.69$ & $4.63\pm0.01$ & $5.88\pm0.08$ & 2.5 \\
SN2020dyu & 17.77 & $8900\pm400$ & $11.18\pm0.69$ & $4.45\pm0.01$ & $5.63\pm0.07$ & 2.2 \\
SN2020fqv & 1.91 & $17900\pm2400$ & $3.11\pm0.43$ & $6.1418\pm0.0002$ & $9.3\pm0.9$ & 1.9 \\
SN2020fqv & 2.55 & $16800\pm1600$ & $3.45\pm0.33$ & $5.6175\pm0.0002$ & $8.3\pm0.5$ & 1.9 \\
SN2020fqv & 3.05 & $15500\pm1400$ & $3.79\pm0.35$ & $2.8475\pm0.0002$ & $5.9\pm0.5$ & 1.8 \\
SN2020fqv & 3.54 & $15000\pm1400$ & $3.98\pm0.4$ & $2.9042\pm0.0002$ & $5.7\pm0.5$ & 1.9 \\
SN2020fqv & 4.54 & $14200\pm1200$ & $4.35\pm0.42$ & $3.1293\pm0.0002$ & $5.6\pm0.4$ & 2.0 \\
SN2020fqv & 5.03 & $13500\pm1300$ & $4.64\pm0.51$ & $3.1804\pm0.0002$ & $5.3\pm0.4$ & 2.4 \\
SN2020fqv & 5.53 & $13000\pm1200$ & $4.89\pm0.52$ & $3.1423\pm0.0002$ & $5.1\pm0.3$ & 2.2 \\
SN2020fqv & 9.5 & $10700\pm600$ & $6.56\pm0.47$ & $2.9044\pm0.0002$ & $4.15\pm0.1$ & 1.3 \\
SN2020fqv & 11.48 & $10300\pm500$ & $6.94\pm0.5$ & $2.789\pm0.0002$ & $3.95\pm0.08$ & 1.4 \\
SN2020fqv & 14.46 & $10000\pm600$ & $7.35\pm0.65$ & $1.9183\pm0.0002$ & $3.8\pm0.2$ & 1.9 \\
SN2020fqv & 17.44 & $9300\pm800$ & $7.98\pm1.0$ & $1.7931\pm0.0002$ & $3.3\pm0.2$ & 4.2 \\
SN2020fqv & 19.42 & $9000\pm700$ & $8.3\pm0.94$ & $1.7104\pm0.0002$ & $3.2\pm0.1$ & 3.2 \\
SN2020fqv & 23.39 & $8800\pm700$ & $8.5\pm0.96$ & $1.2422\pm0.0002$ & $3.1\pm0.2$ & 2.8 \\
SN2020fqv & 26.87 & $8300\pm600$ & $9.16\pm1.04$ & $1.2153\pm0.0002$ & $2.8\pm0.1$ & 2.8 \\
SN2020jfo & 1.4 & $19000\pm400$ & $1.74\pm0.05$ & $1.508\pm0.002$ & $2.86\pm0.05$ & 0.8 \\
SN2020jfo & 4.61 & $12700\pm300$ & $3.3\pm0.13$ & $1.584\pm0.001$ & $2.09\pm0.02$ & 3.1 \\
SN2020jfo & 5.48 & $11700\pm300$ & $3.7\pm0.14$ & $1.504\pm0.001$ & $1.89\pm0.01$ & 3.5 \\
SN2020jfo & 7.0 & $10400\pm200$ & $4.29\pm0.15$ & $1.294\pm0.001$ & $1.578\pm0.008$ & 3.2 \\
SN2020jfo & 7.66 & $10000\pm200$ & $4.45\pm0.16$ & $1.249\pm0.001$ & $1.516\pm0.008$ & 3.2 \\
SN2020jfo & 9.9 & $9000\pm200$ & $5.14\pm0.22$ & $1.0609\pm0.0009$ & $1.288\pm0.008$ & 4.6 \\
SN2020jfo & 10.89 & $8400\pm200$ & $5.59\pm0.27$ & $0.9904\pm0.0009$ & $1.21\pm0.009$ & 5.1 \\
SN2020jfo & 18.99 & $5900\pm200$ & $10.54\pm1.16$ & $0.5617\pm0.0007$ & $0.99\pm0.04$ & 11.7 \\
SN2020jfo & 20.63 & $5700\pm300$ & $10.95\pm1.5$ & $0.5169\pm0.0007$ & $0.95\pm0.04$ & 13.8 \\
SN2020jfo & 27.8 & $5100\pm300$ & $13.61\pm2.37$ & $0.4242\pm0.0005$ & $0.93\pm0.07$ & 18.5 \\
SN2020jfo & 32.12 & $4800\pm300$ & $15.29\pm2.9$ & $0.3911\pm0.0005$ & $0.94\pm0.08$ & 20.0 \\
SN2020jfo & 37.79 & $4600\pm300$ & $16.74\pm3.7$ & $0.3521\pm0.0004$ & $1.0\pm0.1$ & 22.0 \\
SN2020jfo & 43.46 & $4900\pm300$ & $15.06\pm2.74$ & $0.2012\pm0.0003$ & $0.93\pm0.08$ & 2.5 \\
SN2020lfn & 1.44 & $26700\pm1800$ & $3.58\pm0.24$ & $15.25\pm0.03$ & $47.0\pm5.0$ & 2.6 \\
SN2020lfn & 2.3 & $22900\pm2100$ & $4.55\pm0.43$ & $17.51\pm0.03$ & $41.0\pm5.0$ & 6.5 \\
SN2020lfn & 3.9 & $18400\pm1400$ & $6.16\pm0.58$ & $18.22\pm0.03$ & $32.0\pm2.0$ & 8.4 \\
SN2020lfn & 5.43 & $15900\pm900$ & $7.48\pm0.54$ & $16.75\pm0.03$ & $25.8\pm0.8$ & 5.6 \\
SN2020lfn & 6.15 & $14300\pm600$ & $8.49\pm0.49$ & $15.03\pm0.02$ & $21.5\pm0.4$ & 3.9 \\
SN2020lfn & 9.21 & $11900\pm200$ & $10.84\pm0.33$ & $12.3\pm0.02$ & $16.2\pm0.1$ & 1.2 \\
SN2020lfn & 9.65 & $11400\pm200$ & $11.48\pm0.34$ & $11.97\pm0.02$ & $15.54\pm0.1$ & 1.1 \\
SN2020lfn & 11.15 & $10100\pm100$ & $13.34\pm0.34$ & $9.89\pm0.02$ & $12.83\pm0.06$ & 0.8 \\
SN2020lfn & 11.71 & $10400\pm200$ & $12.92\pm0.4$ & $10.77\pm0.02$ & $13.84\pm0.08$ & 1.0 \\
SN2020lfn & 14.13 & $9000\pm100$ & $15.81\pm0.36$ & $9.0\pm0.01$ & $11.78\pm0.05$ & 0.5 \\
SN2020lfn & 15.62 & $8600\pm200$ & $16.92\pm0.65$ & $6.089\pm0.009$ & $11.1\pm0.1$ & 0.6 \\
SN2020lfn & 25.23 & $7000\pm200$ & $20.15\pm1.33$ & $3.973\pm0.006$ & $7.16\pm0.1$ & 1.8 \\
SN2020lfn & 28.32 & $7600\pm200$ & $17.11\pm0.99$ & $3.903\pm0.009$ & $7.01\pm0.09$ & 0.5 \\
SN2020mst & 1.46 & $19700\pm1400$ & $3.31\pm0.33$ & $5.78\pm0.01$ & $11.7\pm0.6$ & 2.0 \\
SN2020mst & 2.37 & $20200\pm900$ & $3.46\pm0.2$ & $6.74\pm0.02$ & $14.1\pm0.6$ & 1.0 \\
SN2020mst & 3.31 & $17600\pm500$ & $4.24\pm0.16$ & $7.7\pm0.01$ & $12.9\pm0.3$ & 0.9 \\
SN2020mst & 8.06 & $12600\pm600$ & $6.47\pm0.41$ & $5.9\pm0.02$ & $7.9\pm0.1$ & 2.0 \\
SN2020mst & 10.98 & $11300\pm500$ & $7.51\pm0.49$ & $5.46\pm0.01$ & $7.04\pm0.1$ & 2.7 \\
SN2020mst & 11.73 & $10600\pm500$ & $8.2\pm0.59$ & $5.05\pm0.01$ & $6.49\pm0.09$ & 2.8 \\
SN2020mst & 13.39 & $10200\pm500$ & $8.62\pm0.67$ & $4.92\pm0.01$ & $6.32\pm0.09$ & 2.8 \\
SN2020nif & 1.88 & $19800\pm600$ & $4.09\pm0.14$ & $9.32\pm0.01$ & $18.6\pm0.5$ & 1.3 \\
SN2020nif & 3.32 & $15900\pm300$ & $5.86\pm0.16$ & $9.97\pm0.01$ & $15.5\pm0.2$ & 1.2 \\
SN2020nif & 4.12 & $14400\pm200$ & $6.98\pm0.16$ & $10.52\pm0.01$ & $15.0\pm0.1$ & 1.0 \\
SN2020nif & 7.59 & $11100\pm200$ & $10.4\pm0.38$ & $10.035\pm0.01$ & $12.37\pm0.07$ & 2.8 \\
SN2020nif & 7.94 & $10900\pm200$ & $10.71\pm0.36$ & $9.775\pm0.009$ & $12.02\pm0.06$ & 2.4 \\
SN2020nif & 8.79 & $10400\pm200$ & $11.5\pm0.47$ & $9.797\pm0.009$ & $11.89\pm0.07$ & 3.3 \\
SN2020nif & 11.14 & $9300\pm200$ & $13.64\pm0.62$ & $9.186\pm0.008$ & $11.05\pm0.07$ & 4.7 \\
SN2020nif & 11.15 & $9300\pm200$ & $13.65\pm0.62$ & $9.18\pm0.008$ & $11.04\pm0.07$ & 4.7 \\
SN2020nif & 11.8 & $9100\pm200$ & $14.15\pm0.61$ & $8.702\pm0.008$ & $10.54\pm0.06$ & 4.4 \\
SN2020nif & 14.15 & $8200\pm200$ & $16.88\pm1.13$ & $7.273\pm0.007$ & $9.9\pm0.1$ & 8.5 \\
SN2020nif & 14.84 & $6000\pm300$ & $29.0\pm4.1$ & $5.057\pm0.005$ & $8.5\pm0.4$ & 22.5 \\
SN2020nif & 16.24 & $7600\pm200$ & $18.96\pm1.17$ & $6.589\pm0.006$ & $9.3\pm0.1$ & 7.2 \\
SN2020nif & 16.67 & $7000\pm200$ & $22.13\pm1.86$ & $6.21\pm0.006$ & $9.2\pm0.2$ & 12.4 \\
SN2020nyb & 1.24 & $20100\pm2400$ & $2.1\pm0.35$ & $2.241\pm0.005$ & $5.0\pm0.5$ & 4.8 \\
SN2020nyb & 1.25 & $20100\pm2400$ & $2.1\pm0.35$ & $2.241\pm0.005$ & $5.0\pm0.5$ & 4.8 \\
SN2020nyb & 2.49 & $16600\pm800$ & $2.71\pm0.21$ & $2.242\pm0.005$ & $3.9\pm0.1$ & 1.6 \\
SN2020nyb & 3.3 & $15500\pm600$ & $3.02\pm0.18$ & $2.234\pm0.005$ & $3.59\pm0.07$ & 1.1 \\
SN2020nyb & 3.83 & $14900\pm600$ & $3.22\pm0.21$ & $2.282\pm0.004$ & $3.51\pm0.07$ & 1.6 \\
SN2020nyb & 4.67 & $13500\pm400$ & $3.65\pm0.17$ & $2.133\pm0.004$ & $3.08\pm0.04$ & 1.0 \\
SN2020nyb & 7.19 & $11000\pm200$ & $4.95\pm0.15$ & $1.911\pm0.004$ & $2.52\pm0.02$ & 0.6 \\
SN2020nyb & 8.07 & $10000\pm200$ & $5.75\pm0.19$ & $1.694\pm0.004$ & $2.42\pm0.02$ & 0.4 \\
SN2020nyb & 8.98 & $9500\pm100$ & $6.24\pm0.13$ & $1.553\pm0.004$ & $2.27\pm0.01$ & 0.1 \\
SN2020nyb & 9.67 & $9100\pm700$ & $6.63\pm0.86$ & $1.588\pm0.004$ & $2.35\pm0.06$ & 3.2 \\
SN2020nyb & 10.52 & $9600\pm900$ & $6.07\pm0.83$ & $0.932\pm0.004$ & $2.2\pm0.1$ & 0.9 \\
SN2020nyb & 12.14 & $9200\pm500$ & $6.36\pm0.55$ & $0.845\pm0.002$ & $2.05\pm0.06$ & 0.5 \\
SN2020pni & 0.65 & $17500\pm900$ & $2.39\pm0.19$ & $1.979\pm0.003$ & $3.7\pm0.1$ & 2.6 \\
SN2020pni & 2.12 & $20600\pm900$ & $3.75\pm0.19$ & $8.438\pm0.01$ & $17.9\pm0.8$ & 3.2 \\
SN2020pni & 3.82 & $17800\pm600$ & $5.33\pm0.22$ & $11.43\pm0.01$ & $20.1\pm0.5$ & 2.5 \\
SN2020pni & 4.28 & $17200\pm500$ & $5.66\pm0.22$ & $11.64\pm0.01$ & $19.8\pm0.4$ & 2.3 \\
SN2020pni & 6.62 & $13700\pm300$ & $7.46\pm0.26$ & $9.76\pm0.01$ & $14.0\pm0.1$ & 1.7 \\
SN2020pni & 9.63 & $11100\pm200$ & $9.45\pm0.35$ & $7.59\pm0.008$ & $10.01\pm0.07$ & 2.3 \\
SN2020pni & 10.55 & $10700\pm200$ & $9.94\pm0.4$ & $7.048\pm0.007$ & $9.28\pm0.07$ & 2.6 \\
SN2020pni & 14.27 & $8800\pm300$ & $12.87\pm0.83$ & $5.461\pm0.006$ & $7.32\pm0.09$ & 6.3 \\
SN2020pni & 16.55 & $8100\pm300$ & $14.04\pm1.01$ & $4.354\pm0.005$ & $6.12\pm0.1$ & 6.5 \\
SN2020pni & 17.8 & $7600\pm300$ & $15.47\pm1.19$ & $4.036\pm0.005$ & $5.8\pm0.1$ & 6.9 \\
SN2020pni & 19.75 & $7100\pm300$ & $16.73\pm1.63$ & $3.345\pm0.004$ & $5.2\pm0.1$ & 8.4 \\
SN2020pni & 23.4 & $7100\pm400$ & $15.73\pm1.77$ & $2.745\pm0.004$ & $4.5\pm0.1$ & 6.9 \\
SN2020pni & 25.66 & $7000\pm600$ & $15.68\pm2.63$ & $2.126\pm0.003$ & $4.2\pm0.1$ & 9.0 \\
SN2020pni & 29.58 & $6800\pm600$ & $15.74\pm2.81$ & $1.805\pm0.003$ & $3.6\pm0.1$ & 8.9 \\
SN2020pni & 31.08 & $6700\pm500$ & $15.41\pm2.44$ & $1.771\pm0.003$ & $3.3\pm0.1$ & 9.6 \\
SN2020pqv & 1.7 & $23500\pm1900$ & $2.91\pm0.24$ & $7.67\pm0.01$ & $19.0\pm2.0$ & 4.1 \\
SN2020pqv & 2.56 & $19100\pm1000$ & $3.73\pm0.23$ & $7.14\pm0.01$ & $13.5\pm0.6$ & 2.8 \\
SN2020pqv & 3.42 & $18800\pm1200$ & $3.89\pm0.3$ & $7.28\pm0.01$ & $13.6\pm0.8$ & 4.7 \\
SN2020pqv & 4.01 & $18400\pm1200$ & $4.02\pm0.32$ & $7.47\pm0.01$ & $13.6\pm0.7$ & 5.1 \\
SN2020pqv & 6.66 & $12400\pm600$ & $6.56\pm0.46$ & $5.845\pm0.008$ & $7.7\pm0.1$ & 4.5 \\
SN2020pqv & 11.13 & $10700\pm400$ & $8.14\pm0.5$ & $5.189\pm0.01$ & $6.59\pm0.08$ & 2.4 \\
SN2020pqv & 13.25 & $9700\pm200$ & $9.47\pm0.38$ & $4.429\pm0.008$ & $5.69\pm0.04$ & 0.9 \\
SN2020pqv & 15.05 & $9000\pm200$ & $10.48\pm0.4$ & $3.811\pm0.007$ & $5.01\pm0.04$ & 0.6 \\
SN2020pqv & 16.91 & $8700\pm300$ & $10.67\pm0.56$ & $3.404\pm0.006$ & $4.54\pm0.04$ & 1.0 \\
SN2020pqv & 18.7 & $8500\pm400$ & $11.03\pm0.82$ & $3.11\pm0.007$ & $4.23\pm0.05$ & 1.4 \\
SN2020pqv & 23.45 & $7500\pm600$ & $12.99\pm1.91$ & $1.996\pm0.004$ & $3.7\pm0.1$ & 2.2 \\
SN2020qvw & 2.62 & $21400\pm1000$ & $4.33\pm0.22$ & $14.75\pm0.02$ & $32.0\pm2.0$ & 1.0 \\
SN2020qvw & 2.64 & $20900\pm700$ & $4.45\pm0.18$ & $14.13\pm0.02$ & $28.0\pm0.9$ & 1.1 \\
SN2020qvw & 3.71 & $18300\pm300$ & $4.95\pm0.11$ & $11.36\pm0.02$ & $19.7\pm0.3$ & 0.5 \\
SN2020qvw & 8.01 & $11400\pm300$ & $8.03\pm0.31$ & $6.4\pm0.02$ & $7.95\pm0.07$ & 0.9 \\
SN2020ufx & 1.75 & $20800\pm1100$ & $5.5\pm0.35$ & $19.7\pm0.03$ & $41.0\pm2.0$ & 1.7 \\
SN2020ufx & 2.76 & $20500\pm1300$ & $5.74\pm0.41$ & $20.45\pm0.03$ & $41.0\pm3.0$ & 3.3 \\
SN2020ufx & 5.93 & $14300\pm500$ & $8.77\pm0.44$ & $15.84\pm0.03$ & $22.6\pm0.4$ & 1.8 \\
SN2020ufx & 11.53 & $9900\pm400$ & $13.67\pm0.92$ & $9.9\pm0.02$ & $12.8\pm0.2$ & 2.1 \\
SN2020ufx & 13.61 & $10000\pm400$ & $13.29\pm0.8$ & $9.78\pm0.02$ & $12.6\pm0.1$ & 0.9 \\
SN2020ufx & 15.21 & $9400\pm500$ & $14.11\pm1.13$ & $8.59\pm0.02$ & $11.2\pm0.2$ & 1.4 \\
SN2020uim & 1.62 & $26700\pm1300$ & $1.6\pm0.08$ & $3.091\pm0.005$ & $9.5\pm0.6$ & 1.0 \\
SN2020uim & 2.6 & $21000\pm900$ & $2.08\pm0.1$ & $2.743\pm0.005$ & $6.0\pm0.3$ & 1.7 \\
SN2020uim & 3.12 & $18600\pm800$ & $2.39\pm0.11$ & $2.799\pm0.005$ & $5.1\pm0.2$ & 1.9 \\
SN2020uim & 4.15 & $16900\pm500$ & $2.65\pm0.1$ & $2.478\pm0.004$ & $4.13\pm0.09$ & 1.3 \\
SN2020uim & 5.14 & $15100\pm400$ & $2.99\pm0.11$ & $2.184\pm0.004$ & $3.3\pm0.06$ & 1.4 \\
SN2020uim & 10.9 & $10200\pm300$ & $4.91\pm0.25$ & $1.52\pm0.003$ & $1.93\pm0.02$ & 1.7 \\
SN2020uim & 12.72 & $10900\pm800$ & $4.51\pm0.42$ & $0.998\pm0.002$ & $2.1\pm0.1$ & 1.4 \\
SN2020uim & 15.01 & $9900\pm400$ & $5.16\pm0.33$ & $0.914\pm0.002$ & $1.83\pm0.05$ & 0.5 \\
SN2020xhs & 2.67 & $17700\pm900$ & $2.59\pm0.19$ & $2.664\pm0.005$ & $4.8\pm0.2$ & 2.0 \\
SN2020xhs & 3.9 & $13400\pm500$ & $3.63\pm0.18$ & $1.585\pm0.004$ & $3.06\pm0.08$ & 0.4 \\
SN2020xhs & 5.28 & $11300\pm300$ & $4.63\pm0.16$ & $0.954\pm0.003$ & $2.56\pm0.05$ & 0.1 \\
SN2020xhs & 16.28 & $7900\pm600$ & $8.16\pm1.02$ & $0.87\pm0.004$ & $1.93\pm0.05$ & 0.6 \\
SN2020xva & 2.0 & $19900\pm1300$ & $1.95\pm0.18$ & $1.877\pm0.004$ & $4.1\pm0.2$ & 2.6 \\
SN2020xva & 3.65 & $15600\pm500$ & $2.63\pm0.15$ & $1.709\pm0.003$ & $2.87\pm0.06$ & 1.4 \\
SN2020xva & 3.71 & $15600\pm500$ & $2.64\pm0.15$ & $1.707\pm0.003$ & $2.86\pm0.06$ & 1.4 \\
SN2020xva & 4.53 & $14900\pm400$ & $2.81\pm0.14$ & $1.673\pm0.003$ & $2.7\pm0.04$ & 0.9 \\
SN2020xva & 6.57 & $12900\pm200$ & $3.44\pm0.07$ & $1.598\pm0.003$ & $2.34\pm0.01$ & 0.2 \\
SN2020xva & 10.17 & $9300\pm300$ & $5.55\pm0.33$ & $1.246\pm0.003$ & $1.62\pm0.02$ & 1.2 \\
SN2020xva & 12.36 & $8400\pm300$ & $6.42\pm0.4$ & $1.087\pm0.003$ & $1.45\pm0.02$ & 1.4 \\
SN2020xva & 12.37 & $8400\pm300$ & $6.43\pm0.4$ & $1.087\pm0.003$ & $1.45\pm0.02$ & 1.4 \\
SN2020xva & 14.02 & $8100\pm600$ & $6.99\pm0.88$ & $0.798\pm0.002$ & $1.47\pm0.05$ & 1.6 \\
SN2020xva & 18.13 & $7800\pm500$ & $7.46\pm0.77$ & $0.588\pm0.001$ & $1.46\pm0.05$ & 0.8 \\
SN2021apg & 2.21 & $20300\pm1000$ & $2.6\pm0.15$ & $3.99\pm0.006$ & $8.3\pm0.4$ & 2.6 \\
SN2021apg & 3.15 & $17400\pm900$ & $3.12\pm0.2$ & $3.619\pm0.006$ & $6.3\pm0.2$ & 3.8 \\
SN2021apg & 4.06 & $15900\pm600$ & $3.39\pm0.21$ & $3.593\pm0.006$ & $5.5\pm0.1$ & 2.4 \\
SN2021apg & 7.51 & $12100\pm800$ & $4.7\pm0.45$ & $2.328\pm0.006$ & $3.6\pm0.1$ & 2.1 \\
SN2021apg & 14.12 & $8400\pm400$ & $7.92\pm0.73$ & $1.659\pm0.004$ & $2.34\pm0.04$ & 1.6 \\
SN2021apg & 18.99 & $8400\pm900$ & $8.0\pm1.43$ & $0.7406\pm0.0009$ & $2.3\pm0.2$ & 2.2 \\
SN2021ibn & 1.99 & $32800\pm1500$ & $2.75\pm0.12$ & $14.48\pm0.02$ & $63.0\pm5.0$ & 0.7 \\
SN2021ibn & 2.54 & $27800\pm1500$ & $3.32\pm0.18$ & $14.14\pm0.02$ & $47.0\pm4.0$ & 1.4 \\
SN2021ibn & 8.11 & $13400\pm400$ & $8.2\pm0.37$ & $10.7\pm0.02$ & $15.0\pm0.2$ & 2.2 \\
SN2021ibn & 10.33 & $10800\pm100$ & $10.67\pm0.21$ & $8.39\pm0.02$ & $10.8\pm0.04$ & 0.4 \\
SN2021ibn & 11.32 & $10500\pm200$ & $10.77\pm0.42$ & $7.42\pm0.01$ & $9.66\pm0.08$ & 1.5 \\
SN2021skn & 1.47 & $26000\pm1400$ & $2.88\pm0.19$ & $8.62\pm0.01$ & $27.0\pm2.0$ & 0.8 \\
SN2021skn & 2.46 & $19500\pm600$ & $4.14\pm0.17$ & $9.27\pm0.01$ & $17.7\pm0.5$ & 1.6 \\
SN2021skn & 3.36 & $17000\pm500$ & $4.91\pm0.21$ & $8.9\pm0.01$ & $14.5\pm0.3$ & 2.0 \\
SN2021skn & 4.49 & $15600\pm400$ & $5.37\pm0.18$ & $8.32\pm0.01$ & $12.5\pm0.2$ & 1.3 \\
SN2021skn & 6.97 & $12500\pm200$ & $6.93\pm0.21$ & $6.61\pm0.01$ & $8.49\pm0.05$ & 1.1 \\
SN2021skn & 9.4 & $10500\pm200$ & $8.57\pm0.32$ & $5.597\pm0.008$ & $6.77\pm0.04$ & 1.5 \\
SN2021skn & 12.06 & $9100\pm200$ & $10.17\pm0.3$ & $4.159\pm0.01$ & $5.12\pm0.03$ & 0.5 \\
SN2021yja & 2.37 & $22900\pm1700$ & $2.23\pm0.23$ & $2.573\pm0.004$ & $9.8\pm0.7$ & 1.1 \\
SN2021yja & 2.59 & $22400\pm1800$ & $2.31\pm0.27$ & $2.59\pm0.004$ & $9.6\pm0.7$ & 1.3 \\
SN2021yja & 3.08 & $18800\pm1400$ & $2.96\pm0.35$ & $2.542\pm0.004$ & $7.9\pm0.3$ & 1.6 \\
SN2021yja & 3.58 & $17300\pm800$ & $3.38\pm0.27$ & $2.516\pm0.004$ & $7.3\pm0.2$ & 0.8 \\
SN2021yja & 5.57 & $14800\pm400$ & $4.21\pm0.23$ & $3.364\pm0.004$ & $6.24\pm0.08$ & 1.1 \\
SN2021yja & 6.07 & $14500\pm400$ & $4.37\pm0.26$ & $3.32\pm0.004$ & $6.09\pm0.08$ & 1.4 \\
SN2021yja & 6.57 & $14100\pm400$ & $4.56\pm0.27$ & $3.255\pm0.004$ & $5.89\pm0.08$ & 1.4 \\
SN2021yja & 7.06 & $13400\pm400$ & $4.91\pm0.33$ & $3.157\pm0.004$ & $5.61\pm0.08$ & 1.8 \\
SN2021yja & 7.56 & $12700\pm500$ & $5.33\pm0.44$ & $3.052\pm0.003$ & $5.35\pm0.1$ & 2.9 \\
SN2021yja & 8.06 & $12500\pm300$ & $5.42\pm0.31$ & $2.97\pm0.003$ & $5.23\pm0.07$ & 1.4 \\
SN2021yja & 16.02 & $8500\pm100$ & $9.38\pm0.38$ & $2.485\pm0.002$ & $3.37\pm0.03$ & 2.7 \\
SN2021yja & 17.51 & $9000\pm700$ & $6.81\pm1.34$ & $2.089\pm0.002$ & $2.65\pm0.09$ & 52.2 \\
SN2021yja & 20.49 & $7500\pm500$ & $9.02\pm1.87$ & $1.739\pm0.002$ & $2.3\pm0.1$ & 59.5 \\
SN2021yja & 24.97 & $6400\pm400$ & $12.03\pm2.54$ & $1.37\pm0.001$ & $2.1\pm0.1$ & 54.4 \\
SN2021yja & 25.47 & $6200\pm400$ & $12.55\pm2.71$ & $1.34\pm0.001$ & $2.0\pm0.2$ & 55.4 \\
SN2021yja & 27.95 & $5700\pm400$ & $15.03\pm3.43$ & $1.226\pm0.001$ & $2.0\pm0.2$ & 57.7 \\
SN2021yja & 32.43 & $5400\pm500$ & $16.35\pm4.24$ & $1.084\pm0.001$ & $1.9\pm0.2$ & 54.0 \\
\hline
\hline
\hline
\enddata
\tablenotetext{a}{A full version of this table is made available through the journal website.}
\tablenotetext{b}{A 0.1 mag systematic error was adopted for the fitting.}
\end{deluxetable*}



==> tab_bb_trunc.tex <==
\begin{deluxetable*}{lcccccccc}
\label{tab:bb_trunc}
\centering
\tablecaption{Early-time blackbody fits of SNe included in this work (truncated)}
\tablewidth{34pt} 
\tablehead{\colhead{SN} & \colhead{t [rest-frame days]} & \colhead{$\rm T_{eff}\ [K]$} & \colhead{$\rm R_{BB}\ [10^{14} \rm cm]$ } & \colhead{$\rm L_{pseudo}\ [10^{42} \rm erg\ \rm s^{-1}]$} & \colhead{$\rm L_{pseudo,extrap}\  [10^{42} \rm erg\ \rm s^{-1}]$}& \colhead{$\chi^{2}/dof$}  } 
\tabletypesize{\scriptsize} 
\startdata
SN2018cxn & 1.6 & $23500\pm1500$ & $2.15\pm0.16$ & $3.749\pm0.009$ & $10.0\pm0.7$ & 1.4 \\
SN2018cxn & 2.19 & $20800\pm1400$ & $2.58\pm0.22$ & $3.767\pm0.009$ & $8.7\pm0.5$ & 2.2 \\
SN2018cxn & 5.6 & $12700\pm600$ & $5.3\pm0.42$ & $3.497\pm0.007$ & $5.1\pm0.1$ & 2.0 \\
SN2018cxn & 9.59 & $10500\pm300$ & $6.82\pm0.34$ & $2.827\pm0.007$ & $3.88\pm0.04$ & 0.6 \\
SN2018dfc & 1.58 & $22000\pm800$ & $4.31\pm0.2$ & $13.18\pm0.02$ & $31.0\pm1.0$ & 1.0 \\
SN2018dfc & 3.19 & $17000\pm500$ & $5.99\pm0.25$ & $12.46\pm0.02$ & $21.7\pm0.4$ & 1.0 \\
SN2018dfc & 4.1 & $15000\pm300$ & $6.92\pm0.21$ & $10.69\pm0.02$ & $17.1\pm0.2$ & 0.5 \\
SN2018dfc & 5.03 & $13300\pm200$ & $8.19\pm0.29$ & $9.88\pm0.02$ & $14.7\pm0.1$ & 0.5 \\
SN2018fif & 1.22 & $20600\pm1500$ & $1.68\pm0.14$ & $1.671\pm0.003$ & $3.7\pm0.3$ & 2.7 \\
SN2018fif & 1.25 & $20100\pm1100$ & $1.73\pm0.12$ & $1.646\pm0.003$ & $3.5\pm0.2$ & 2.1 \\
SN2018fif & 2.1 & $15600\pm500$ & $2.7\pm0.15$ & $1.851\pm0.003$ & $3.08\pm0.06$ & 1.6 \\
SN2018fif & 2.65 & $15100\pm700$ & $2.87\pm0.21$ & $1.813\pm0.003$ & $2.96\pm0.07$ & 2.9 \\
SN2018fif & 4.57 & $12000\pm600$ & $4.22\pm0.3$ & $1.976\pm0.003$ & $2.65\pm0.05$ & 3.6 \\
SN2018fif & 6.15 & $11200\pm600$ & $4.86\pm0.42$ & $2.041\pm0.003$ & $2.68\pm0.05$ & 4.4 \\
SN2018fif & 6.17 & $11100\pm600$ & $4.87\pm0.42$ & $2.042\pm0.003$ & $2.68\pm0.05$ & 4.4 \\
SN2018fif & 7.31 & $10600\pm600$ & $5.33\pm0.46$ & $2.037\pm0.003$ & $2.66\pm0.04$ & 4.2 \\
SN2018fif & 8.33 & $10000\pm500$ & $5.86\pm0.49$ & $1.997\pm0.004$ & $2.6\pm0.04$ & 3.5 \\
\hline
\hline
\enddata
\tablenotetext{a}{A full version of this table is made available through the journal website.}
\tablenotetext{b}{A 0.1 mag systematic error was adopted for the fitting.}
\end{deluxetable*}



==> tab_colors.tex <==
\begin{deluxetable*}{clccccccc}
\centering
\label{tab:colors}
\tablecaption{SNe II early-time colors}
\tablewidth{34pt} 
\tablehead{\colhead{t [rest-frame days]} &   \colhead{Filter} &   \colhead{$\lambda_{piv}$ [\AA]} &       \colhead{$W_{eff}$ [\AA]} &  \colhead{Mean $m_{\lambda}-m_{r}$ [mag]} &  \colhead{STD [mag]} &  \colhead{Bluest color [mag]} &  \colhead{Reddest color [mag]} &  \colhead{$N_{SN}$}} 
\tabletypesize{\scriptsize} 
\startdata
       1 &   UVW2 &        2055 &    305 &               -0.70 &       0.27 &      -1.13 &      -0.49 &     5 \\
       1 &   UVM2 &        2246 &    259 &               -0.70 &       0.30 &      -1.12 &      -0.32 &     5 \\
       1 &   UVW1 &        2580 &    397 &               -0.57 &       0.25 &      -0.97 &      -0.35 &     5 \\
       1 &      u &        3467 &    352 &               -0.53 &       0.20 &      -0.82 &      -0.34 &     5 \\
       1 &      g &        4702 &    641 &               -0.24 &       0.09 &      -0.43 &      -0.05 &    18 \\
       1 &      i &        7489 &    767 &                0.27 &       0.15 &       0.14 &       0.60 &     6 \\
       \hline
       2 &   UVW2 &        2055 &    305 &               -0.67 &       0.27 &      -1.30 &      -0.18 &    23 \\
       2 &   UVM2 &        2246 &    259 &               -0.64 &       0.28 &      -1.23 &      -0.02 &    22 \\
       2 &   UVW1 &        2580 &    397 &               -0.59 &       0.22 &      -1.17 &      -0.20 &    23 \\
       2 &      u &        3467 &    352 &               -0.59 &       0.21 &      -0.95 &      -0.12 &    23 \\
       2 &      g &        4702 &    641 &               -0.27 &       0.11 &      -0.44 &       0.06 &    30 \\
       2 &      i &        7489 &    767 &                0.27 &       0.23 &       0.08 &       0.98 &    22 \\
       \hline
       3 &   UVW2 &        2055 &    305 &               -0.33 &       0.30 &      -0.89 &       0.24 &    30 \\
       3 &   UVM2 &        2246 &    259 &               -0.37 &       0.30 &      -0.94 &       0.14 &    30 \\
       3 &   UVW1 &        2580 &    397 &               -0.36 &       0.24 &      -0.93 &       0.12 &    30 \\
       3 &      u &        3467 &    352 &               -0.45 &       0.24 &      -1.05 &       0.16 &    30 \\
       3 &      g &        4702 &    641 &               -0.18 &       0.12 &      -0.45 &       0.10 &    31 \\
       3 &      i &        7489 &    767 &                0.23 &       0.21 &       0.00 &       0.93 &    25 \\
       \hline
       4 &   UVW2 &        2055 &    305 &               -0.01 &       0.35 &      -0.57 &       0.68 &    29 \\
       4 &   UVM2 &        2246 &    259 &               -0.13 &       0.31 &      -0.71 &       0.39 &    29 \\
       4 &   UVW1 &        2580 &    397 &               -0.17 &       0.28 &      -0.73 &       0.29 &    29 \\
       4 &      u &        3467 &    352 &               -0.34 &       0.25 &      -1.01 &       0.28 &    30 \\
       4 &      g &        4702 &    641 &               -0.14 &       0.10 &      -0.39 &       0.02 &    31 \\
       4 &      i &        7489 &    767 &                0.23 &       0.15 &      -0.02 &       0.80 &    24 \\
       \hline
       5 &   UVW2 &        2055 &    305 &                0.31 &       0.35 &      -0.29 &       0.98 &    27 \\
       5 &   UVM2 &        2246 &    259 &                0.13 &       0.29 &      -0.45 &       0.62 &    26 \\
       5 &   UVW1 &        2580 &    397 &                0.01 &       0.22 &      -0.45 &       0.47 &    28 \\
       5 &      u &        3467 &    352 &               -0.25 &       0.21 &      -0.51 &       0.41 &    28 \\
       5 &      g &        4702 &    641 &               -0.12 &       0.09 &      -0.28 &       0.10 &    29 \\
       5 &      i &        7489 &    767 &                0.21 &       0.10 &      -0.00 &       0.42 &    23 \\
\hline
\enddata
\tablenotetext{a}{}
\end{deluxetable*}

==> tab_sn_list.tex <==
\begin{deluxetable*}{llcccccccl}
\centering
\label{tab:sn_list}
\tablecaption{List of 34 SNe included in this study}
\tablewidth{34pt} 
\tablehead{\colhead{SN} &\colhead{ZTF ID} & \colhead{$\alpha$ (J2000)} & \colhead{$\delta$ (J2000)} & \colhead{z} & \colhead{$d^{a}$ [Mpc]} & \colhead{$t_{ND}$ [JD]} & \colhead{$t_{exp}$ [JD]} & \colhead{$\tau_{flash}^{b}$ [days]} & \colhead{Reference$^{c}$}} 
\tabletypesize{\scriptsize} 
\startdata
SN\,2018cxn & ZTF18abckutn & 237.026897 & 55.714855 & 0.0401 & 186.6 & 2458289.7490 & $2458289.76\pm0.01$ & $<0.0$ & [1] \\
SN\,2018dfc & ZTF18abeajml & 252.032360 & 24.304095 & 0.0365 & 170.0 & 2458302.7103 & $2458303.8\pm0.009$ & $6.2\pm2.8$ & [1] \\
SN\,2018fif & ZTF18abokyfk & 2.360629 & 47.354083 & 0.0172 & 76.5 & 2458349.8973 & $2458350.874\pm0.002$ & $1.6\pm1.0$ & [1.2]\\
SN\,2019eoh & ZTF19aatqzim & 195.955635 & 38.289155 & 0.0501 & 229.6 & 2458601.7817 & $2458606.683\pm0.031$ & $<0.0$ & [3] \\
SN\,2019gmh & ZTF19aawgxdn & 247.763189 & 41.153961 & 0.0307 & 141.3 & 2458633.8250 & $2458634.324\pm0.444$ & $<1.4$ & [3] \\
SN\,2019nvm & ZTF19abqhobb & 261.411100 & 59.446730 & 0.0181 & 86.4 & 2458713.7416 & $2458714.69\pm0.007$ & $1.9\pm1.0$ & [3,4] \\
SN\,2019omp & ZTF19abrlvij & 260.142987 & 51.632780 & 0.0450 & 206.9 & 2458717.7910 & $2458718.713\pm0.0$ & $<0.0$ & [3] \\
SN\,2019oxn & ZTF19abueupg & 267.803290 & 51.382550 & 0.0200 & 90.3 & 2458723.7895 & $2458724.342\pm0.129$ & $<0.4$ & [3] \\
SN\,2019ozf & ZTF19abulrfa & 279.817010 & 54.287872 & 0.0480 & 221.2 & 2458723.7900 & $2458724.728\pm0.005$ & $<0.0$ & [3] \\
SN\,2019ust & ZTF19acryurj & 13.593396 & 31.670182 & 0.0220 & 96.0 & 2458799.8053 & $2458800.04\pm0.177$ & $5.0\pm0.5$ & [3] \\
SN\,2019wzx & ZTF19aczlldp & 37.782326 & 4.311291 & 0.0275 & 124.9 & 2458833.7282 & $2458835.506\pm0.092$ & $<1.1$ & [11] \\
SN\,2020cxd & ZTF20aapchqy & 261.621953 & 71.094063 & 0.0039 & 23.7 & 2458896.0296 & $2458896.671\pm0.671$ & $<2.4$ & [5,6] \\
SN\,2020dyu & ZTF20aasfhia & 184.913047 & 33.040393 & 0.0500 & 230.7 & 2458911.9254 & $2458912.814\pm0.021$ & $<0.0$ & [3] \\
SN\,2020fqv & ZTF20aatzhhl & 189.138576 & 11.231654 & 0.0075 & 15.0 & 2458936.9007 & $2458939.43\pm0.16$ & $<0.9$ & [7] \\
SN\,2020jfo & ZTF20aaynrrh & 185.460355 & 4.481697 & 0.0052 & 14.7 & 2458971.7751 & $2458975.231\pm0.424$ & $<0.5$ & [8] \\
SN\,2020lfn & ZTF20abccixp & 246.737033 & 20.245906 & 0.0440 & 202.2 & 2458995.8154 & $2458996.701\pm0.018$ & $4.2\pm1.5$ & [3] \\
SN\,2020mst & ZTF20abfcdkj & 281.793965 & 60.496802 & 0.0590 & 274.0 & 2459012.8161 & $2459013.689\pm0.067$ & $<0.1$ & [3] \\
SN\,2020nif & ZTF20abhjwvh & 196.057282 & -10.351002 & 0.0104 & 50.5 & 2459021.7334 & $2459023.783\pm0.765$ & $<0.9$ & [11] \\
SN\,2020nyb & ZTF20abjonjs & 29.783900 & 86.676205 & 0.0155 & 72.1 & 2459026.9709 & $2459033.849\pm0.014$ & $<0.0$ & [11] \\
SN\,2020pni & ZTF20ablygyy & 225.958184 & 42.114032 & 0.0169 & 83.2 & 2459045.7542 & $2459046.638\pm0.004$ & $5.0\pm1.0$ & [9] \\
SN\,2020pqv & ZTF20abmoakx & 220.498180 & 8.462724 & 0.0338 & 160.2 & 2459046.7104 & $2459048.646\pm0.023$ & $5.2\pm2.5$ & [3] \\
SN\,2020qvw & ZTF20abqkaoc & 250.983335 & 77.879897 & 0.0500 & 230.7 & 2459065.8438 & $2459066.222\pm0.417$ & $<0.6$ & [11] \\
SN\,2020afdi & ZTF20abqwkxs & 224.868111 & 73.898678 & 0.0239 & 110.9 & 2459069.7995 & $2459070.277\pm0.341$ & $1.3\pm0.5$ & [3] \\
SN\,2020ufx & ZTF20acedqis & 322.652706 & 24.673752 & 0.0500 & 230.7 & 2459116.8338 & $2459117.752\pm0.015$ & $4.9\pm1.0$ & [3] \\
SN\,2020uim & ZTF20acfdmex & 28.188740 & 36.623160 & 0.0185 & 80.5 & 2459117.8602 & $2459118.823\pm0.0$ & $<0.1$ & [3] \\
SN\,2020xhs & ZTF20acknpig & 30.742868 & 45.020286 & 0.0244 & 106.6 & 2459138.8669 & $2459138.936\pm0.301$ & $<1.8$ & [3] \\
SN\,2020xva & ZTF20aclvtnk & 263.035128 & 53.653989 & 0.0240 & 108.7 & 2459141.7258 & $2459142.69\pm0.69$ & $<1.0$ & [3] \\
SN\,2020aavm & ZTF20acrinvz & 116.681975 & 18.113551 & 0.0450 & 227.2 & 2459168.9788 & $2459169.935\pm0.746$ & $<1.0$ & [11] \\
SN\,2020abue & ZTF20acvjlev & 121.084598 & 56.302082 & 0.0280 & 126.9 & 2459188.0078 & $2459189.663\pm0.118$ & $<0.2$ & [11] \\
SN\,2020acbm & ZTF20acwgxhk & 40.074159 & 2.427067 & 0.0217 & 93.1 & 2459192.7093 & $2459193.654\pm0.022$ & $<0.1$ & [11] \\
SN\,2021apg & ZTF21aafkwtk & 205.330192 & 24.495531 & 0.0269 & 128.4 & 2459228.0064 & $2459230.722\pm0.186$ & $<1.2$ & [11] \\
SN\,2021ibn & ZTF21aasfseg & 132.558710 & 37.026990 & 0.0442 & 197.2 & 2459306.7862 & $2459307.252\pm0.295$ & $<0.4$ & [11] \\
SN\,2021skn & ZTF21abjcjmc & 246.204167 & 39.734653 & 0.0297 & 139.5 & 2459397.8203 & $2459398.735\pm0.743$ & $<1.1$ & [11] \\
SN\,2021yja & ZTF21acaqdee & 51.088215 & -21.565626 & 0.0053 & 22.6 & 2459459.4000 & $2459464.4\pm0.06$ & $<2.3$ & [10] \\
\hline
\enddata
\tablenotetext{a}{Corrected for Virgo, Great Attractor, and Shapley supercluster infall.}
\tablenotetext{b}{In rest-frame days, calculated using the last spectrum showing flash features or by taking the first spectrum as an upper limit.}
\tablenotetext{c}{[1] \cite{Bruch2021}, [2] \cite{Soumagnac2020}, [3] \cite{bruch2022}, [4] \cite{Vallely2021}, [5] \cite{Yang2021}, [6] \cite{Valerin2022}, [7] \cite{Tinyanont2022}, [8] \cite{Sollerman2021}, [9] \cite{Terreran2022}}, [10] \cite{Hosseinzadeh2022}, [11] TNS classification reports: \cite{Perley_tns_19,Hiramatsu2020,Perley_tns_2020,Dahiwale2020c,Weil2020_tns,Dahiwale2020d,Pessi2020_tns,Delgado2021_tns,Deckers2021_tns,Siebert_2021_tns}.
\tablenotetext{d}{This table is available in machine-readable format.}

\end{deluxetable*}
